Distributed Personalized Empirical Risk Minimization

This paper advocates a new paradigm Personalized Empirical Risk Minimization (PERM) to facilitate learning from heterogeneous data sources without imposing stringent constraints on computational resources shared by participating devices. In PERM, we aim to learn a distinct model for each client by learning who to learn with and personalizing the aggregation of local empirical losses by effectively estimating the statistical discrepancy among data distributions, which entails optimal statistical accuracy for all local distributions and overcomes the data heterogeneity issue. To learn personalized models at scale, we propose a distributed algorithm that replaces the standard model averaging with model shuffling to simultaneously optimize PERM objectives for all devices. This also allows us to learn distinct model architectures (e.g., neural networks with different numbers of parameters) for different clients, thus confining underlying memory and compute resources of individual clients. We rigorously analyze the convergence of the proposed algorithm and conduct experiments that corroborate the effectiveness of the proposed paradigm.

==> acknowledge.tex <==
\section*{Acknowledgement}
We would like to thank Mohammad Mahdi Kamani for his help on conducting the experiments. We would also like to thank an anonymous reviewer from ICML 2021 for pointing out an issue of the assumption on $\phi$ in the previous version of this manuscript.

==> addinional_experiemnts.tex <==
In addition to the synthetic dataset discussed in the main body, we run experiments on the EMNIST dataset~\cite{caldas2018leaf}, which is naturally distributed in a federated setting. In this case, we chose 50 clients and use a 2-layer MLP model, each with 200 neurons. We compare the PERM algorithm with the localized model in FedAvg and perFedAvg~\cite{fallah2020personalized}. As it can be seen in Figure~\ref{fig:emnist}, PERM can learn a better personalized model by attending to each client's data according to the similarity of the data distribution between clients. The learned values of $\balpha$ show that the clients are learning from each others' data, and not focused on their own data only. This signifies that the distribution of data among clients in this dataset is not highly heterogeneous. Note that, since we are using a subset of clients in the EMNIST dataset for the training (only 50 clients for 100 rounds of communication), the results would be sub-optimal. Nonetheless, the experiments are designed to show the effectiveness of different algorithms. 
\begin{figure}[t!]
  \centering
  \begin{subfigure}[b]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/emnist_acc.pdf}
    \caption{Personalized Accuracy}
    \label{fig:emnist-acc}
  \end{subfigure}
  \hspace{20pt}
  \begin{subfigure}[b]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/emnist_loss.pdf}
    \caption{Personalized Loss}
    \label{fig:emnist-loss}
  \end{subfigure}
  \caption{Comparative Analysis of Personalization methods, including our single-loop PERM algorithm, localized FedAvg, and perFedAg, with EMNIST dataset. The disparity in personalized accuracy and loss highlights PERM's capability in leveraging relevant client correlations.}
  \label{fig:emnist}\vspace{-2mm}
\end{figure}
\begin{figure}[t!]
  \centering
  \begin{minipage}{0.5\textwidth}
    \includegraphics[width=0.75\textwidth]{Figures/alpha_emnist.pdf}
  \end{minipage}%
  % \hspace{1pt}
  \begin{minipage}{0.4\textwidth}
    \captionof{figure}{The heat map of the learned $\bm{\alpha}$ values for the PERM algorithms. The weights signify that clients mutually benefiting from one another's data, which also highlight that the distribution of data is not significantly heterogeneous in this dataset.}
    \label{app:fig:alpha}
  \end{minipage} \vspace{-5mm}
\end{figure}
\subsection{The effectiveness of learned mixture weights}
To show the effectiveness of two-stage PERM algorithm, as well as the effects of heterogeneity on distribution of data among clients on the learned weights $\balpha$ in the algorithm, we run this algorithm on MNIST dataset. We use 50 clients, and the model is an MLP, similar to the EMNIST experiment. In this case, once we distribute the data randomly across clients (homogeneous) and once only allocating 1 class per client (highly heterogeneous). As it can be seen from Figure~\ref{fig:mnist}, when the data distribution is homogeneous the learned values of $\balpha$ as diffused across clients. However, when the data is highly heterogeneous, the learned $\balpha$ values will be highly sparse, indicating that each client is mostly learning from its own data and some other clients with partial distribution similarity.

\begin{figure}[t!]
  \centering
  \begin{subfigure}[b]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/alpha_mnist_iid.pdf}
    \caption{Homogeneous distribution}
    \label{fig:mnist_iid}
  \end{subfigure}
  \hspace{20pt}
  \begin{subfigure}[b]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/alpha_mnist_noniid.pdf}
    \caption{Highly heterogeneous distribution}
    \label{fig:mnist_noniid}
  \end{subfigure}
  \caption{Comparing the performance of two-stage PERM algorithm in learning $\alpha$ values on heterogeneous and homogeneous data distributions. WE use MNIST dataset across 50 clients with homogeneous and heterogeneous distributions.}
  \label{fig:mnist}\vspace{-2mm}
\end{figure}

==> algorithm.tex <==

\begin{algorithm2e}[t]
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\DontPrintSemicolon
    \caption{\texttt{Local (S)GD}}
	\label{algorithm: GD}
 
    	\textbf{Input:} Synchronization gap $\tau$ , Number of iterations $T$.  Initialization network parameter $\bm{W}(0) \sim \mathcal{N}(0,2/m\bm{I})$ and $\bm{v} \sim \mathcal{N}(0,  \bm{I}/d)$
	\\
 
	\textbf{parallel} \For{$i = 1,...,K$}{
	 
	 \For{$t = 1,...,T$}{
  
 	   \algemph{antiquewhite}{0.85}{       ${\bm{W}}^{(i)}(t+1) = {\bm{W}}^{(i)}(t) - \eta \nabla_{\bm{W}}      L_i\left({\bm{W}}^{(i)}(t)\right) $ \qquad  \# Local GD  }\\   
 	   \algemph{blizzardblue}{0.85}{
 	   Sample a data $(\Tilde{\bm{x}}, \Tilde{y})$ uniformly from $S_i$.\\
 	    Compute $\bm{G}_i^{(t)} = n \nabla_{\bm{W}}      \ell\left({\bm{W}}^{(i)}(t);\Tilde{\bm{x}}, \Tilde{y} \right)$.\\
 	 ${\bm{W}}^{(i)}(t+1) = {\bm{W}}^{(i)}(t) - \eta \bm{G}_i^{(t)} $  \qquad \qquad \qquad \quad \# Local SGD  \\   }
	 \If{$t$ divides $\tau$}{
	        all nodes send their local parameter ${\bm{W}}^{(i)}(t+1)$ to server.\\
           $ \bm{W}(t+1) = \frac{1}{K}\sum_{i=1}^K {\bm{W}}^{(i)}(t+1)$;\\
 	         
 	        send $ \bm{W}(t+1)$ to all nodes to update their local models. \\
 	        each client initializes its local models: $\bm{W}^{(i)}(t+1)= \bm{W}(t+1)$.} 
	 } 
	
  }
 
 
\end{algorithm2e} 



% \begin{algorithm2e}[t]
% 	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
% 	\DontPrintSemicolon
%     \caption{\texttt{Local SGD}}
% 	\label{algorithm: SGD}
 
%     	\textbf{Input:} Synchronization gap $\tau$, Number of iterations $T$. Initialization network parameter $\bm{W}(0) \sim \mathcal{N}(0,2/m\bm{I})$ and $\bm{v} \sim \mathcal{N}(0,  \bm{I}/d)$
% 	\\
 
% 	\textbf{parallel} \For{$i = 1,...,K$}{
	 
% 	 \For{$t = 1,...,T$}{
  
%  	 {Sample a data $(\Tilde{\bm{x}}, \Tilde{y})$ uniformly from $S_i$.\\
%  	 Compute $\bm{G}_i^{(t)} = n \nabla_{\bm{W}}      \ell\left({\bm{W}}^{(i)}(t);\Tilde{\bm{x}}, \Tilde{y} \right)$.\\
%  	 ${\bm{W}}^{(i)}(t+1) = {\bm{W}}^{(i)}(t) - \eta \bm{G}_i^{(t)} $   \\   }
% 	 \If{$t$ divides $\tau$}{
% 	        all nodes send their local parameter ${\bm{W}}^{(i)}(t+1)$ to server.\\
%           $ \bm{W}(t+1) = \frac{1}{K}\sum_{i=1}^K {\bm{W}}^{(i)}(t+1)$;\\
 	         
%  	        send $ \bm{W}(t+1)$ to all nodes to update their local models. \\
%  	        each client initializes its local models: $\bm{W}^{(i)}(t+1)= \bm{W}(t+1)$.} 
% 	 } 
	
%   }
 
 
% \end{algorithm2e} 


==> discussion.tex <==
\section{Discussion and Future Works}\label{sec: discussion}
In this paper, we proved
that both Local GD and Local SGD that are originally proposed for communication efficient network training can achieve global minima of the training loss for over-parameterized
deep ReLU networks. We make the first theoretical trial on the analysis of Local (S)GD on training Deep ReLU network, but we do not claim that our results, e.g., number of required neurons and dependency on the number of layers, are optimal in any sense. A number of future works/improvements are still exciting to explore.


\noindent\textbf{Tightening the condition on the number of neurons.}~In both Local GD and SGD bound,we require the number of neurons to have a heavy dependency on $n$, worse than the single machine case. We are aware of some recent works~\cite{noy2021convergence,nguyen2020global,nguyen2021proof} that have significantly reduced the  number of required neuron, and  we believe incorporating their results can also improve our theory.

\noindent\textbf{Extension of analysis to other federated optimization methods.} To further reduce the harm caused by multiple local updates, a line of recent studies proposed alternative methods to reduce the  local model deviation~\cite{karimireddy2019scaffold,yuan2020federated}. Establishing the  convergence of these variants on deep non-smooth networks is another valuable research direction.  
 
 
\noindent\textbf{Extension to other neural network architectures.} In this paper we only consider simple ReLU forward feed neural network, but as shown in the prior works~\cite{allen2019convergence,zou2020global}, single machine SGD can optimize more complicated neural network like CNN, ResNet or RNN as well. Hence, one natural future work is to extend our analysis on Local SGD to those neural network model.

==> generalization.tex <==
\section{Generalization of PERM}

We may wish to bound
\begin{align*}
  \E\left[\cL_i(\hat{h}^{\textrm{PERM}})\right] \leq  \E\left[\sum_{j=1}^N \hat{\balpha}_i(j)\widehat{\cL}_j(\hat{h}^{\textrm{PERM}})\right]  +...
\end{align*}
where the expectation is taken over the training sets $S_1,..,S_N$, and randomness of algorithm.

==> related.tex <==
\section{Additional Related Works}
\paragraph{Data-aware distributed optimization}{Many prior works establish .... In contrast to these previous studies, our focus is on designing an algorithm that .....

Moreover, we put a particular emphasis on
}


\paragraph{System-aware  distributed optimization}{and model-heterogeneous There is a lengthy literatures}

\paragraph{Multiple source domain adaptation}{Our setting  from a theoretical perspective relates to , the seminal work of~\cite{ben2010theory} considers a setting
where labeled data from many source tasks and a target task is available. They show that minimizing
a weighted combination of the source and target empirical risks leads to the best result.}

